Search for $CP$-Violating Neutrino Nonstandard Interactions with the NOvA Experiment

This Letter reports a search for charge-parity ($CP$) symmetry violating nonstandard interactions (NSI) of neutrinos with matter using the NOvA Experiment, and examines their effects on the determination of the standard oscillation parameters. Data from $\nu_{\mu}(\bar{\nu}_{\mu})\rightarrow\nu_{\mu}(\bar{\nu}_{\mu})$ and $\nu_{\mu}(\bar{\nu}_{\mu})\rightarrow\nu_{e}(\bar{\nu}_{e})$ oscillation channels are used to measure the effect of the NSI parameters $\varepsilon_{e\mu}$ and $\varepsilon_{e\tau}$. With 90% CL the magnitudes of the NSI couplings are constrained to be $|\varepsilon_{e\mu}| \, \lesssim 0.3$ and $|\varepsilon_{e\tau}| \, \lesssim 0.4$. A degeneracy at $|\varepsilon_{e\tau}| \, \approx 1.8$ is reported, and we observe that the presence of NSI limits sensitivity to the standard $CP$ phase $\delta_{\tiny\text{CP}}$.

==> ShortCuts.tex <==
%New Commands (Math)
\newcommand {\nux}{$\nu_{x}$}
\newcommand {\delm}{$\Delta m^{2}$}
\newcommand {\delmatm}{$\Delta m^2_{32}$}
\newcommand {\thetaatm}{$\theta_{23}$}
\newcommand {\sqsin}{$\sin^{2} 2\theta$}
\newcommand {\loe}{$L/E$}
\newcommand {\loenu}{$L/E_{\nu}$}
\newcommand {\loevis}{$L/E_{vis}$}
\newcommand {\sqchi}{$\chi^{2}$}
\newcommand {\ccnm}{\mbox{CC-$\nu_\mu$}}
\newcommand {\ccne}{\mbox{CC-$\nu_e$}}
\newcommand {\nmflvr}{\mbox{$\nu_\mu$\ flavor}}
\newcommand {\nmFLVR}{\mbox{$\nu_\mu$-FLAVOR}}
\newcommand {\neflvr}{\mbox{$\nu_e$-flavor}}
\newcommand {\dlmval}[1]{\ensuremath{\mbox{$\Delta m^{2} = #1$} \
\mbox{eV}^{2}}}
\newcommand {\evsq}{$\mbox{eV}^{2}$}

\newcommand {\degr}{\mbox{$\,^{\circ}$}}

\newcommand{\etal}{{\em et al.}\bs}
\newcommand{\ie}{{\em i.e.}\bs}
\newcommand{\eg}{{\em e.g.}\bs}
\newcommand{\cf}{{\em cf.}\bs}
\newcommand{\h}{\hfill{}\\}
\newcommand{\hl}{\hline}
\newcommand{\hs}[1]{\hspace{#1}}
\newcommand{\bs}{\hspace{5.0pt}}
\newcommand{\ls}{\hspace*{50pt}}
\newcommand{\bl}{\hspace{3.0pt}}
\newcommand{\s}{\mb{s}}
\newcommand{\tnn}{\mbox{$\tau_{n\overline{n}}\ $}}
\newcommand{\Tnn}{\mbox{$T_{n\overline{n}}$}}
\newcommand{\TA}{\mbox{$T_{A}$}\bs}
\newcommand{\TAn}{\mbox{$T_{A}$}}
\newcommand{\Tnty}{\mbox{$T_{A, n_{90}}$}\bl}
\newcommand{\TR}{\mbox{$T_{R}$}\bs}
\newcommand{\TRn}{\mbox{$T_{R}$}}
\newcommand{\enn}{\mbox{$\epsilon_{n\overline{n}}$}}

\newcommand{\lequ}[1]{\lefteqn{#1}}
\newcommand{\mulc}[3]{\multicolumn{#1}{#2}{#3}}
\newcommand{\rbx}[2]{\raisebox{#1}{#2}}
\newcommand{\mb}[1]{\mbox{#1}}
\newcommand{\cp}[1]{\caption{#1}}
\newcommand{\vs}{\vspace{-0.15in}}

\newcommand{\frejus}{Fr\'{e}jus\hs{0.2cm}}
\newcommand{\frejusn}{Fr\'{e}jus}
\newcommand{\pnet}{\mbox{$P_{net}$}\bs}
\newcommand{\pnetn}{\mbox{$P_{net}$}}
\newcommand{\evis}{\mbox{$E_{vis}$}\bs}
\newcommand{\evisn}{\mbox{$E_{vis}$}}

%\newcommand{\n}{$\overline{\mb{\rm n}}$\hs{0.2cm}}       % anti-neutron
\newcommand{\nn}{${\rm n}\overline{\rm n}$\hs{0.2cm}}    % neutron,anti-neutron
\newcommand{\nN}{\mbox{$\rm {\overline{n}N}$}\hs{0.2cm}} % anti-neutron + nucleon
\newcommand{\nNn}{\mbox{$\rm {\overline{n}N}$}}
\newcommand{\NN}{\mbox{$\rm {\overline{N}N}$}\hs{0.2cm}} % anti-nucleon + nucleon
\newcommand{\pmm}{$\pm$}                                 % plus and minus in math mode

\newcommand{\neut}{\mbox{$\nu$}}                         % nu
%\newcommand{\numu}{\mbox{$\nu_{\mu}$}}                   % nu_mu
%\newcommand{\nue}{\mbox{$\nu_{e}$}}                      % nu_e
%\newcommand{\nutau}{\mbox{$\nu_{\tau}$}}                 % nu_tau
\newcommand{\anu}{\mbox{$\overline{\nu}$}}               % anu
\newcommand{\anue}{\mbox{$\overline{\nu}_{e}$}}          % anu_e
\newcommand{\anumu}{\mbox{$\overline{\nu}_{\mu}$}}       % anu_mu

\newcommand{\pn}{\mbox{$\pi$}}                           % pion
\newcommand{\pipm}{$\pi^{\pm}$}                     % pion plus minus
\newcommand{\pip}{\mbox{$\pi^{+}$}}                      % pi plus
\newcommand{\pim}{\mbox{$\pi^{-}$}}                      % pi minus
\newcommand{\piz}{\mbox{$\pi^{0}$}}                      % pi zero
\newcommand{\spip}{\mbox{$\scriptscriptstyle\pi^{+}$}}   % pi plus small
\newcommand{\spim}{\mbox{$\scriptscriptstyle\pi^{-}$}}   % pi minus small
\newcommand{\m}{$\mu$}                                   % muon
\newcommand{\mupm}{$\mu^{\pm}$}                     % muon plus minus
\newcommand{\mup}{\mbox{$\mu^{+}$}}                      % mu plus
\newcommand{\mum}{\mbox{$\mu^{-}$}}                      % mu minus
\newcommand{\del}{\delta}                                % delta
\newcommand{\g}{\mbox{$\gamma$}}                         % gamma
\newcommand{\epm}{$e^{\pm}$}   %electron plus minus
\newcommand{\eplus}{$e^{+}$}    %electron plus
\newcommand{\eminus}{$e^{-}$}   % electron minus

%\newcommand{\ket}[1]{\left|#1\right\rangle}
\newcommand{\num}{\numu}
\newcommand{\numbar}{\bar\numu}
\newcommand{\nus}{\nu_s}
\newcommand{\nut}{\nu_{\tau}}

\newcommand{\Uo}[1]{{|U_{#1}|^2}}
\newcommand{\Ut}[2]{{|U_{#1}|^2|U_{#2}|^2}}

